Toward Efficient Language Model Pretraining and Downstream Adaptation via Self-Evolution: A Case Study on SuperGLUE

This technical report briefly describes our JDExplore d-team's Vega v2 submission on the SuperGLUE leaderboard. SuperGLUE is more challenging than the widely used general language understanding evaluation (GLUE) benchmark, containing eight difficult language understanding tasks, including question answering, natural language inference, word sense disambiguation, coreference resolution, and reasoning. [Method] Instead of arbitrarily increasing the size of a pretrained language model (PLM), our aim is to 1) fully extract knowledge from the input pretraining data given a certain parameter budget, e.g., 6B, and 2) effectively transfer this knowledge to downstream tasks. To achieve goal 1), we propose self-evolution learning for PLMs to wisely predict the informative tokens that should be masked, and supervise the masked language modeling (MLM) process with rectified smooth labels. For goal 2), we leverage the prompt transfer technique to improve the low-resource tasks by transferring the knowledge from the foundation model and related downstream tasks to the target task. [Results] According to our submission record (Oct. 2022), with our optimized pretraining and fine-tuning strategies, our 6B Vega method achieved new state-of-the-art performance on 4/8 tasks, sitting atop the SuperGLUE leaderboard on Oct. 8, 2022, with an average score of 91.3.

==> [TechReport2022] Vega-V2/all_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[h]
\caption{\textbf{Results of Top-10 models on SuperGLUE leaderboard} (\url{https://super.gluebenchmark.com/leaderboard}), on October 8, 2022.
}
\label{tab:allrank}
\centering \small
\scalebox{0.85}{
\begin{tabular}{clcccccccccccc}
\toprule
\multirow{2}{*}{\bf $\#$Rank} & \multicolumn{1}{c}{\multirow{2}{*}{\bf Model}} & \textbf{BoolQ} & \multicolumn{2}{c}{\bf CB} & \textbf{COPA}  & \multicolumn{2}{c}{\bf MultiRC} & \multicolumn{2}{c}{\bf ReCoRD} & \textbf{RTE}  & \textbf{WiC}  & \textbf{WSC}   & \multirow{2}{*}{\bf Score} \\ \cmidrule{3-13}
                      & \multicolumn{1}{c}{}                       & Acc   & F1         & Acc       & Acc   & F1           & EM           & F1           & Acc.        & Acc  & Acc  & Acc   &                        \\ \midrule
1                     & Vega v2 (Ours)                                & 90.5  & 98.6       & 99.2      & 99.4  & 88.2         & 62.4         & 94.4         & 93.9        & 96.0 & 77.4 & 98.6  & 91.3                   \\
2                     & ST-MoE-32B                                 & 92.4  & 96.9       & 98.0      & 99.2  & 89.6         & 65.8         & 95.1         & 94.4        & 93.5 & 77.7 & 96.6  & 91.2                   \\
3                     & Turing NLR v5                              & 92.0  & 95.9       & 97.6      & 98.2  & 88.4         & 63.0         & 96.4         & 95.9        & 94.1 & 77.1 & 97.3  & 90.9                   \\
4                     & ERNIE 3.0                                  & 91.0  & 98.6       & 99.2      & 97.4  & 88.6         & 63.2         & 94.7         & 94.2        & 92.6 & 77.4 & 97.3  & 90.6                   \\
5                     & PaLM 540B                                  & 91.9  & 94.4       & 96.0      & 99.0  & 88.7         & 63.6         & 94.2         & 93.3        & 94.1 & 77.4 & 95.9  & 90.4                   \\
6                     & T5+UKG, Single Model        & 91.4  & 95.8       & 97.6      & 98.0  & 88.3         & 63.0         & 94.2         & 93.5        & 93.0 & 77.9 & 96.6  & 90.4                   \\
7                     & DeBERTa/ TuringNLRv4                       & 90.3  & 95.7       & 97.6      & 98.4  & 88.2         & 63.7         & 94.5         & 94.1        & 93.2 & 77.5 & 95.9  & 90.3                   \\
8                     & SuperGLUE Human Baselines                  & 89.0  & 95.8       & 98.9      & 100.0 & 81.8         & 51.9         & 91.7         & 91.3        & 93.6 & 80.0 & 100.0 & 89.8                   \\
9                     & T5                                         & 91.2  & 93.9       & 96.8      & 94.8  & 88.1         & 63.3         & 94.1         & 93.4        & 92.5 & 76.9 & 93.8  & 89.3                   \\
10                    & Frozen T5 1.1 + SPoT                       & 91.1  & 95.8       & 97.6      & 95.6  & 87.9         & 61.9         & 93.3         & 92.4        & 92.9 & 75.8 & 93.8  & 89.2                \\
\bottomrule
\end{tabular}
}
\end{table*}

==> [TechReport2022] Vega-V2/main_results.tex <==
\begin{table*}[!t]
\caption{\textbf{Results obtained on the SuperGLUE test sets}, which are scored by the SuperGLUE evaluation server. We obtained the results from \url{https://super.gluebenchmark.com} on October 8, 2022. The best results (except the those of human baselines) are shown in bold.}
\label{table_main}
\centering
\scalebox{0.76}{
\begin{tabular}{lcccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Model}}    & BoolQ & \multicolumn{2}{c}{CB} & COPA  & \multicolumn{2}{c}{MultiRC} & \multicolumn{2}{c}{ReCoRD} & RTE  & WiC  & WSC   & \multirow{2}{*}{Score} \\ \cmidrule{2-12}
                          & Acc   & F1         & Acc       & Acc   & F1           & EM           & F1           & Acc.        & Acc  & Acc  & Acc   &                        \\ \midrule \midrule
\textbf{SuperGLUE Baselines}       & 79.0  & 84.8       & 90.4      & 73.8  & 70.0         & 24.1         & 72.0         & 71.3        & 79.0 & 69.6 & 64.4  & 71.5                   \\
\textbf{SuperGLUE Human Baselines} & 89.0  & 95.8       & 98.9      & 100.0 & 81.8         & 51.9         & 91.7         & 91.3        & 93.6 & 80.0 & 100.0 & 89.8                   \\ \hdashline
\textbf{PaLM 540B}~\cite{chowdhery2022palm}                 & 91.9  & 94.4       & 96.0      & 99.0  & 88.7         & 63.6         & 94.2         & 93.3        & 94.1 & 77.4 & 95.9  & 90.4                   \\
\textbf{ERNIE 3.0}~\cite{sun2021ernie}                 & 91.0  & 98.6       & \textbf{99.2}      & 97.4  & 88.6         & 63.2         & 94.7         & 94.2        & 92.6 & 77.4 & 97.3  & 90.6                   \\
\textbf{Turing NLR v5}~\cite{bajaj2022metro}             & 92.0  & 95.9       & 97.6      & 98.2  & 88.4         & 63.0         & \textbf{96.4}         & \textbf{95.9}        & 94.1 & 77.1 & 97.3  & 90.9                   \\
\textbf{ST-MoE-32B}~\cite{zoph2202st}                & \textbf{92.4}  & 96.9       & 98.0      & 99.2  & \textbf{89.6}         & \textbf{65.8}         & 95.1         & 94.4        & 93.5 & \textbf{77.7} & 96.6  & 91.2                   \\
\textbf{Vega v2 (Ours)}               & 90.5  & \textbf{98.6}       & \textbf{99.2}      & \textbf{99.4}  & 88.2         & 62.4         & 94.4         & 93.9        & \textbf{96.0} & 77.4 & \textbf{98.6}  & \textbf{91.3}     \\
\bottomrule
\end{tabular}
}
\end{table*}

==> [TechReport2022] Vega-V2/task_descriptions.tex <==
\begin{table*}[t]
\caption{\textbf{Data statistics of different tasks included in SuperGLUE} according to their original paper~\cite{superglue}.  
\textit{WSD} stands for word sense disambiguation, \textit{NLI} is natural language inference, \textit{coref.} is coreference resolution, and \textit{QA} is question answering. For MultiRC, we list the number of total answers for 456/83/166 train/dev/test questions. 
%The metrics for MultiRC are binary F1 on all answer-options and exact match.
}
\centering \small
\begin{tabular}{lrrrlll}
 \toprule
\textbf{Corpus} & \textbf{$|$Train$|$} & \textbf{$|$Dev$|$} & \textbf{$|$Test$|$} & \textbf{Task} & \textbf{Metrics} & \textbf{Text Sources} \\
\midrule 
BoolQ & 9427 & 3270 & 3245 & QA & acc. & Google queries, Wikipedia \\
CB & 250 & 57 & 250 & NLI & acc./F1 & various \\
COPA & 400 & 100 & 500 & QA & acc. & blogs, photography encyclopedia\\
MultiRC & 5100 & 953 & 1800 & QA & F1$_a$/EM & various \\
ReCoRD & 101k & 10k & 10k & QA & F1/EM & news (CNN, Daily Mail) \\
RTE & 2500 & 278 & 300 & NLI & acc. & news, Wikipedia \\
WiC & 6000 & 638 & 1400 & WSD & acc. & WordNet, VerbNet, Wiktionary \\
WSC & 554 & 104 & 146 & coref. & acc. & fiction books \\
\bottomrule
\end{tabular}
\label{tab:tasks}
\end{table*}


==> [TechReport2022] Vega-V2/task_examples.tex <==
\begin{table*}[t]
\caption{\textbf{Task examples from the valid set in SuperGLUE}~\cite{superglue}. \textbf{Bold} text represents part of the example format for each task. Text in \textit{italics} is part of the model input. \underline{\textit{Underlined}} text is specially marked in the input. Text in a \texttt{monospaced font} represents the expected model output.}
\label{tab:examples}
\centering \footnotesize
\begin{tabular}{p{0.005\textwidth}p{0.93\textwidth}}
 \toprule
 \parbox[t]{1mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{{\textbf{BoolQ}}}}} &
\textbf{Passage:} \textit{Barq's -- Barq's is an American soft drink. Its brand of root beer is notable for having caffeine. Barq's, created by Edward Barq and bottled since the turn of the 20th century, is owned by the Barq family but bottled by the Coca-Cola Company. It was known as Barq's Famous Olde Tyme Root Beer until 2012.} \\ & \textbf{Question:} \textit{is barq's root beer a pepsi product} \quad \textbf{Answer:} \texttt{No}\\

\midrule
\parbox[t]{1mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{{\textbf{CB}}}}} &
\textbf{Text:} \textit{B: And yet, uh, I we-, I hope to see employer based, you know, helping out. You know, child, uh, care centers at the place of employment and things like that, that will help out. A: Uh-huh. B: What do you think, do you think we are, setting a trend?} \\ & \textbf{Hypothesis:} \textit{they are setting a trend} \quad \textbf{Entailment:} \texttt{Unknown}\\

\midrule
\parbox[t]{1mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{{\textbf{COPA}}}}} & \textbf{Premise:} \textit{My body cast a shadow over the grass.}\quad
\textbf{Question:} \textit{What’s the CAUSE for this?}\\
&\textbf{Alternative 1:} \textit{The sun was rising.}\quad
\textbf{Alternative 2:} \textit{The grass was cut.}\\
&\textbf{Correct Alternative:} \texttt{1}\\


\midrule
\parbox[t]{1mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{{\textbf{MultiRC}}}}} &
\textbf{Paragraph:} \textit{Susan wanted to have a birthday party. She called all of her friends. She has five friends. Her mom said that Susan can invite them all to the party. Her first friend could not go to the party because she was sick. Her second friend was going out of town. Her third friend was not so sure if her parents would let her. The fourth friend said maybe. The fifth friend could go to the party for sure. Susan was a little sad. On the day of the party, all five friends showed up. Each friend had a present for Susan. Susan was happy and sent each friend a thank you card the next week}\\
& \textbf{Question:} \textit{Did Susan's sick friend recover?} \textbf{Candidate answers:} 
\textit{Yes, she recovered} (\texttt{T}), 
\textit{No} (\texttt{F}), 
\textit{Yes} (\texttt{T}), 
\textit{No, she didn't recover} (\texttt{F}), 
\textit{Yes, she was at Susan's party} (\texttt{T})\\

\midrule
\parbox[t]{1mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{{\textbf{ReCoRD}}}}} & 
\textbf{Paragraph:} \textit{(\underline{CNN}) \underline{Puerto Rico} on Sunday overwhelmingly voted for statehood. But Congress, the only body that can approve new states, will ultimately decide whether the status of the \underline{US} commonwealth changes. Ninety-seven percent of the votes in the nonbinding referendum favored statehood, an increase over the results of a 2012 referendum, official results from the \underline{State Electorcal Commission} show. It was the fifth such vote on statehood. "Today, we the people of \underline{Puerto Rico} are sending a strong and clear message to the \underline{US Congress}  ... and to the world ... claiming our equal rights as \underline{American} citizens, \underline{Puerto Rico} Gov. \underline{Ricardo Rossello} said in a news release. @highlight \underline{Puerto Rico} voted Sunday in favor of \underline{US} statehood}\\
&\textbf{Query} For one, they can truthfully say, ``Don't blame me, I didn't vote for them, '' when discussing the <placeholder> presidency \quad \textbf{Correct Entities:} \texttt{US} \\

\midrule
\parbox[t]{1mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{{\textbf{RTE}}}}} &
\textbf{Text:} \textit{Dana Reeve, the widow of the actor Christopher Reeve, has died of lung cancer at age 44, according to the Christopher Reeve Foundation.}\\
& \textbf{Hypothesis:} \textit{Christopher Reeve had an accident.} \quad
\textbf{Entailment:} \texttt{False}\\

\midrule
\parbox[t]{1mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{{\textbf{WiC}}}}} &
\textbf{Context 1:} \textit{Room and \underline{board}.} \quad
\textbf{Context 2:} \textit{He nailed \underline{boards} across the windows.} \\
& \textbf{Sense match:} \texttt{False}\\

\midrule
\parbox[t]{1mm}{\multirow{1}{*}{\rotatebox[origin=c]{90}{{\textbf{WSC}}}}} & 
\textbf{Text:} \textit{Mark told \underline{Pete} many lies about himself, which Pete included in his book. \underline{He} should have been more truthful.} \quad \textbf{Coreference:} \texttt{False}\vspace{0.25em}\\
\bottomrule
\end{tabular}

\end{table*}

